Knowledge Graph Self-Supervised Rationalization for Recommendation

In this paper, we introduce a new self-supervised rationalization method, called KGRec, for knowledge-aware recommender systems. To effectively identify informative knowledge connections, we propose an attentive knowledge rationalization mechanism that generates rational scores for knowledge triplets. With these scores, KGRec integrates generative and contrastive self-supervised tasks for recommendation through rational masking. To highlight rationales in the knowledge graph, we design a novel generative task in the form of masking-reconstructing. By masking important knowledge with high rational scores, KGRec is trained to rebuild and highlight useful knowledge connections that serve as rationales. To further rationalize the effect of collaborative interactions on knowledge graph learning, we introduce a contrastive learning task that aligns signals from knowledge and user-item interaction views. To ensure noise-resistant contrasting, potential noisy edges in both graphs judged by the rational scores are masked. Extensive experiments on three real-world datasets demonstrate that KGRec outperforms state-of-the-art methods. We also provide the implementation codes for our approach at https://github.com/HKUDS/KGRec.

==> solution_back.tex <==
\section{PRELIMINARIES}
We first introduce concepts as well as notations that will be used in the paper, and formalize our KG-aware recommendation task.

\paratitle{User-Item Interaction Graph.}
Consider a typical recommendation scenario, in which a user set $\mathcal{U}$ and item set $\mathcal{V}$ is given. And $u\in\mathcal{U}$ and $v\in\mathcal{V}$ denote single user and item, respectively. We naturally construct a binary graph $\mathcal{G}_u = \{(u, y_{uv}, v)\}$ from the interactions to denote the collaborative signals between users and items, \ie $y_{uv}=1$ if user $u$ interacted with item $v$, and vice versa.

\paratitle{Knowledge Graph.}
We represent real-world knowledge with a heterogeneous graph with triplets $\mathcal{G}_k = \{(h,r,t)\}$. Particularly, $h,t\in\mathcal{E}$ are knowledge entities and $r\in\mathcal{R}$ represents the semantic relation connecting them, \eg~(\textit{Paris, the capital of, France}). Note that the item set is a proper subset of the entity set: $\mathcal{V}\subset\mathcal{E}$.

\paratitle{Task Formulation.}
For the KG-aware recommendation task, our goal can be formally described as: given a user-item interaction graph $\mathcal{G}_u$ and a knowledge graph $\mathcal{G}_k$, we learn a pairwise rating model as $\mathcal{F}(u,v|\mathcal{G}_u,\mathcal{G}_k,\Theta)$, where $\mathcal{F}$ denotes the model architecture with learnable parameters $\Theta$. The output results in the range $[0,1]$ judges how likely the user $u$ would interact with item $v$.
\section{Methodology}
\label{sec:solution}
\begin{figure*}
    \centering
    \includegraphics[width=0.9\linewidth]{material/model_arc_.pdf}
    \vspace{-0.1in}
    \caption{The overall framework of \model. Attentive knowledge rationalization generates rational scores for KG triplets. Connections with high rational scores are masked and \model~is trained to reconstruct the important connections under relational context. Low-scored KG triplets are considered as noise to be removed for rationales contrastive learning between u-i and KG graphs. Knowledge aggregation for recommendation is also weighted by the rational scores.}
    \label{fig:arch}
    \vspace{-0.15in}
\end{figure*}

In this section, we introduce detailed technical design of our proposed~\model. The overall framework is present in Figure~\ref{fig:arch}.
% Generally, we propose a fundamental attentive rationalization mechanism to weight the importance of each knowledge triplet  (entity, relation, entity). Then, based on the rational scores, we first empower the heterogeneous knowledge aggregation mechanism with dynamic weights to reflect the varying priority of different knowledge triplets. To further denoise the knowledge graph for recommendation and highlight the significant semantics in the KG, we introduce a self-supervision paradigm that includes both generative and contrastive manners. To unify the data augmentation, we build the two tasks on the adaptive masking module. Specifically, for the generative SSL, we mask knowledge triplets that are top attentive and force the model to reconstruct these significant connections. For the contrastive SSL, we follow the attentive scores to drop potential noise in both knowledge graph and u-i graph and let the model learn to align the noise-free consistency between the two graphs by adopting a contrastive learning objective.
\subsection{Attentive Knowledge Rationalization}
To automatically distill important semantics for recommendation from the complex knowledge graph, we consider to learn a rational weighting function that discriminates the rationality of  knowledge triplets. In particular, we rationalize each knowledge triplet based on a learnable graph attention mechanism. Inspired by heterogeneous graph transformer (HGT)~\cite{hgt} that emphasizes heterogeneous relations in graph convolution, given a knowledge triplet $(h,r,t)$, we implement the rational weighting function $f(h,r,t)$ as:
\begin{align}
\label{eq:rational}
    f(h,r,t) =  \frac{\mathbf{e}_h\mathbf{W}^Q \cdot \left(\mathbf{e}_t\mathbf{W}^K \odot \mathbf{e}_r\right)^\trans}{\sqrt{d}}, 
\end{align}
where $\mathbf{e}_h, \mathbf{e}_r, \mathbf{e}_t$ are embeddings for $h,r,t$ separately. $\mathbf{W}^Q, \mathbf{W}^K \in \mathbb{R}^{d\times d}$ are trainable attention weights and $d$ is the hidden dimension. Note we use the element-wise product between the relation $r$ and tail entity $t$ to model the relational context, which is essentially the rotation of entity embedding $\mathbf{e}_t$ to the latent space of relation $r$~\cite{rotate,kgin}. Comprehensively, as trained by labels from the recommendation task, a knowledge triplet with higher rational score $f(h,r,t)$ indicates that it is more conducive to making recommendation decisions. To further make rational scores of knowledge triplets locally comparable across neighbors of the same head entity, we normalize the scores by the number of neighbors $\mathcal{N}_h$ using a softmax function:
\begin{equation}
\label{eq:kg_w}
    \omega(h,r,t) = \frac{\exp\left(f(h,r,t)\right)}{\sum_{(h,r^\prime,t^\prime)\in \mathcal{N}_h}\exp \left(f\left(h,r^\prime,t^\prime\right)\right)}.
\end{equation}

\subsection{Rationalized Heterogeneous Knowledge Aggregation}
\label{sec:kgagg}
A complex knowledge graph usually contains real-world knowledge triplets with the heterogeneity nature. Inspired by~\cite{kgat, kgin, kgcl}, we design a aggregation layer for the knowledge graph that reflects the relational heterogeneity of knowledge triplets. Rationales of knowledge triplets are another key focus for aggregation, which enables dynamic weighting considering the importance of neighbor entities. Therefore, to fulfil the above two aspects, we build the knowledge aggregator by injecting the relational context into entity neighbor embeddings and weight the aggregation by knowledge rational scores:
\begin{equation}
\label{eq:kgagg}
    \mathbf{e}_h^{(l)} = \frac{1}{|\mathcal{N}_h|} \sum_{(h,r,t)\in \mathcal{N}_h}\omega(h,r,t)\mathbf{e}_r\odot\mathbf{e}_t^{(l-1)},
\end{equation}
where $l$ denotes the layer of the aggregator and $\mathcal{N}_h \subseteq \mathcal{G}_k$ is the node-centric sub-graph of first-order neighbors. For the injection of relational context, we keep it consistent with Equation~\ref{eq:rational} as the element-wise product to bridge the gap between aggregation and rational weighting. By performing such aggregation across the whole knowledge graph, we carefully consider contextual relationships between knowledge entities and weight neighbor information for the head entity according to normalized rational scores.

Note that since items are a subset of knowledge entities, we obtain knowledge-aware item representations by aggregation paths $\mathbf{e}_v\leftarrow\mathbf{e}_{t_1}\leftarrow\cdots\leftarrow\mathbf{e}_{t_n}$ on the KG by Equation~\ref{eq:kgagg}. To this end, we consider the role of users on the interaction graph $\mathcal{G}_u$ to model collaborative signals between users and items. Hence, we further generate user embeddings by neighbor aggregation on the user-item interaction graph as:
\begin{equation}
    \mathbf{e}_u^{(l)} = \frac{1}{|\mathcal{N}_u|} \sum_{i\in \mathcal{N}_u}\mathbf{e}_v^{(l-1)},
\end{equation}
where $\mathbf{e}_u, \mathbf{e}_v$ are the user embedding and item embedding, accordingly. Item $v$ is equivalent to a certain entity $h,t$ in the KG.

Here, we can define the final representations of users and entities as the summation of aggregated embeddings from different layers:
\begin{equation}
\label{eq:sum}
    \mathbf{e}_h = f_k(\mathcal{G}_k;h) = \sum_l^L\mathbf{e}_h^{(l)};\  \mathbf{e}_u = f_u(\mathcal{G}_u;u) = \sum_l^L\mathbf{e}_u^{(l)},
\end{equation}
where $L$ is the layer size and $f_*(\cdot;\cdot)$ denotes the function to generate user or entity representations given the input graph and certain instances.
% \vspace{-0.2in}
\subsection{Rational Knowledge Masking and Reconstructing}
\subsubsection{\textbf{Learning to Mask with Rationality}}
As revealed by related works~\cite{transa, kbert, shi2018open}, noisy or irrelevant connections between entities in knowledge graphs can lead to suboptimal representation learning. In knowledge-aware recommendation, the issue can be exacerbated since user and item representations are further interrupted by KG noise~\cite{kgcl, kopra} to derive inaccurate recommendation results. To eliminate the noise effect in KG and distill informative signals that benefit the recommendation task, we propose to highlight important knowledge triplets of high rational scores learned in Equation~\ref{eq:rational} to guarantee better representation learning. 

Recent revisiting studies on masked autoencoders (MAEs)~\cite{he2022masked, feichtenhofer2022masked} point out that it allows the model to better acquire useful implicit semantics by masking important information during training and training the model to recover the missing knowledge. Inspired by this, we design a generative self-supervised learning task in the masking-and-reconstructing manner. Specifically, during each training step, we mask a batch of knowledge triplets in the KG, and reconstruct these relational edges by a generative self-supervised objective. We further require that the masked triplets have globally high rational scores. In other words, we mask knowledge that is important for the recommendation task, and force the model to learn to reconstruct these connections as to highlight useful knowledge.

We first design the criterion to judge the rational importance of knowledge triplets from a global view. Recall that in Equation~\ref{eq:kg_w}, we obtain $\omega(h,r,t)$ that reflects the local importance of the triplet among all edges to the same head entity $h$. The limitation here is that the value of $\omega$ is subject to the degree of the head entity, which makes $\omega$ only locally comparable. To make $\omega$ globally comparable across the whole KG, a simple workaround is to magnify $\omega(h,r,t)$ by the number of its head entity neighbors $|\mathcal{N}_h|$ as:
\begin{equation}
    \gamma(h,r,t) = |\mathcal{N}_h|\cdot \omega(h,r,t) = \frac{|\mathcal{N}_h|\cdot\exp\left(f(h,r,t)\right)}{\sum_{(h,r^\prime,t^\prime)\in \mathcal{N}_h}\exp \left(f\left(h,r^\prime,t^\prime\right)\right)}.
\end{equation}
The intuition behind is that a knowledge triplet with higher rational score after softmax would have a higher relative proportion among neighbors of its head entity $\mathcal{N}_h$. And by multiplying the neighbor size we can make the proportion independent of the number of neighbors, thus globally comparable. To this end, we can select highest valuable knowledge triplets across the whole KG by the value of $\gamma(h,r,t)$. Considering the optimal sampling ability of Gumbel distribution for discrete stochasticity~\cite{gumbel}, we add Gumbel noise to the learned rational scores to improve sampling robustness:
\begin{equation}
    \gamma(h,r,t) = \gamma(h,r,t)-\log\left(-\log(\epsilon)\right);\quad\epsilon\sim\text{Uniform}\left(0,1\right),
\end{equation}
where $\epsilon$ is the random variable sampled from uniform distribution. Then, we generate a set of masked knowledge triplets by selecting the top $k$-highest rational scores in the KG:
\begin{equation}
\label{eq:mk}
    \mathcal{M}_k = \{(h,r,t)|\gamma(h,r,t)\in\text{topk}(\Gamma;k_m)\},
\end{equation}
where $\Gamma$ denotes the distribution of all $\gamma(h,r,t)$. At last, by removing edges $\mathcal{M}_k$ from the knowledge graph $\mathcal{G}_k$, we generate an augmented knowledge graph $\mathcal{G}_k^m$ where triplets of size $k_m$ with important rationales are masked:
\begin{equation}
    \mathcal{G}_k^m = \mathcal{G}_k \setminus \mathcal{M}_k,
\end{equation}
where $\setminus$ denotes the set minus operation.
\subsubsection{\textbf{Reconstructing with Relation-aware Objective}}
To facilitate our model with the capacity to recover important knowledge in a self-supervised manner, the model is fed with entity embeddings generated from the augmented graph $\mathcal{G}_k^m$, and is trained to reconnect the masked knowledge edges. Hence, we first apply the rationalized knowledge aggregation as in Equation~\ref{eq:kgagg} on $\mathcal{G}_k^m$ to generate entity embeddings with a $k_m$ size of rational edges invisible: 
\begin{equation}
    \mathbf{e}_h = f_k(\mathcal{G}_k^m;h);\ \mathbf{e}_t = f_k(\mathcal{G}_k^m;t),
\end{equation}
where $f_k(\cdot)$ is the aggregation function on knowledge graph defined in Equation~\ref{eq:sum}. To this stage, knowledge triplets with important rationales $\mathcal{M}_k$ that are invisible during the aggregation can thus serve as self-supervision labels for reconstructing. Considering rich relational heterogeneity in the KG, we force the label triplets to minimize the following dot-product log-loss as reconstructing important rational connections under relational contexts:
\begin{equation}
\label{eq:mr}
    \mathcal{L}_m = \sum_{(h,r,t)\in \mathcal{M}_k}-\log\left(\sigma\left( \mathbf{e}_h^\trans\cdot\left(\mathbf{e}_t\odot\mathbf{e}_r\right)\right)\right),
\end{equation}
where $\sigma$ denotes the sigmoid activation function.

\subsection{Cross-View Rationales Contrast}
\subsubsection{\textbf{Rationalized Graph Augmentation}}
As aforementioned, the hierarchical rationales for knowledge triplets are results of the connection between the KG and user-involved recommendation labels. To further improve the interpretability of the designed knowledge rationalization modules, inspired by~\cite{kgic,mcclk}, we devise to align knowledge graph representations with collaborative filtering signals for explicit modeling of cross-view rationales. To build debiased contrastive views, we first design to recognize and remove weakly task-related edges that are potentially noise in both graphs. 

For the KG, recall that knowledge triplets with lower rational scores tend to be less contributive to the recommendation task. Therefore, we augment the KG by removing the noisy triplets:
\begin{equation}
    \mathcal{S}_k = \{(h,r,t)|\gamma(h,r,t)\in\text{topk}(-\Gamma;\rho_k)\};\ \mathcal{G}_k^c = \mathcal{G}_k \setminus \mathcal{S}_k,
\end{equation}
where $\gamma, \Gamma$ are the knowledge attentive scores with Gumbel noise, same as in Equation~\ref{eq:mk}. $-\Gamma$ is the negative $\gamma$ values which turns top-k function to calculate least-k. And $\rho_k$ is the hyperparameter that controls the dropout ratio. $\mathcal{G}_k^c$ is the augmented knowledge graph that is debiased from noise with lower rational scores.

As for the u-i interaction graph, we aim to remove noisy interactions that are not conducive to cross-view alignment. In particular, we expect to retain interaction edges that clearly reflect the user's interests and thus can better guide knowledge graph rationalization by cross-view contrasting. Considering that the semantics of item embedding can be affected by its linked knowledge in the KG, we devise to weight each interaction edge by considering the rationales of the knowledge triplets connected to the item. Technically, we calculate the mean value of rational scores for knowledge triplets linked with the item to reflect the noise of the interaction edge:
\begin{equation}
    \phi_v = \text{mean}(\{\gamma(h,r,t)|{h=v\vee t=v}\}).
\end{equation}
Hence, a lower $\phi_v$ indicates that knowledge entities neighboring the item in the KG are relatively less contributive to the recommendation task, causing bias in the item representation. To this stage, we filter our interaction edges with low $\phi_v$ to augment the graph. Here we utilize the multinomial distribution sampling strategy~\cite{huang2022stochastic, li2020federated} to derive more randomized samples for edge dropout to avoid over-fitting on user and item representations. Formally, the process can be defined as:
\begin{equation}
    \phi_v^\prime  = \frac{\exp \phi_v}{\sum_v \exp \phi_v};\ \mathcal{S}_u\sim\text{multinomialNR}(\Phi^\prime;\rho_u),
\end{equation}
where $\phi^\prime$ denotes the probability value of $\phi$ after softmax on all items. $\Phi^\prime$ is the distribution of $\phi^\prime_i$ and $\text{multinomialNR}(\cdot;\cdot)$ is the multinomial distribution without replacement. $\rho_u$ denotes the size of sampled candidates. To this stage, following the previous definition, we can generate the augmented u-i graph as $\mathcal{G}_u^c=\mathcal{G}_u\setminus \mathcal{S}_u$.
\subsubsection{\textbf{Contrastive Learning for Cross-View Rationales.}}
With the augmented knowledge graph and u-i graph, we use different pre-defined aggregators to capture the view-specific node representations for items as the contrastive embeddings. For the u-i interaction view, we utilize the state-of-the-art LightGCN~\cite{he2020lightgcn} module to iteratively capture the high-order information on $\mathcal{G}_u^c$:
\begin{equation}
\mathbf{x}_u^{(l)} = \sum_{v\in\mathcal{N}_u}\frac{\mathbf{x}_v^{(l-1)}}{\sqrt{|\mathcal{N}_u||\mathcal{N}_v|}};\ \mathbf{x}_v^{(l)} = \sum_{u\in\mathcal{N}_v}\frac{\mathbf{x}_u^{(l-1)}}{\sqrt{|\mathcal{N}_u||\mathcal{N}_v|}}.
\end{equation}
And by summing up the representation from all layers, we obtain the final representation as $\mathbf{x}_v^u = \sum_l^L\mathbf{x}_v^{(l)}$.
For the augmented knowledge graph, we adopt the rationalized knowledge aggregation mechanism as defined in Equation~\ref{eq:sum} to generate the knowledge-view item representations:
\begin{equation}
    \mathbf{x}_v^k = f_k(\mathcal{G}_k^c; v).
\end{equation}
Note that $\mathbf{x}_i^u$ and $\mathbf{x}_i^k$ are from different representation spaces of collaborative signals and knowledge signals, we feed them into two different two-layer MLPs to map them into the same latent space:
\begin{equation}
    \mathbf{z}_v^* = \sigma\left(\mathbf{x}_v^{*\trans}\mathbf{W}_1^* + \mathbf{b}_1^*\right)^\trans\mathbf{W}_2^* + \mathbf{b}_2^*,
\end{equation}
where $* = {u,k}$ denotes view-specific representations $\mathbf{z}_v^u$ and $\mathbf{z}_v^k$. $\mathbf{W}, \mathbf{b}$ are learnable weights and bias.

Finally, we adopt a contrastive objective to force the alignment of cross-view item representations. To avoid over-fitting and eliminate the false-negative effect, inspired by~\cite{wang2022swift}, we modify the widely used InfoNCE~\cite{infonce} loss to specify one random sample for each view as the negative. Formally, we define our contrastive loss as:
\begin{equation}
\label{eq:lc}
    \mathcal{L}_c = \sum_{v\in\mathcal{V}}-\log\frac{\exp(s(\mathbf{z}_v^u, \mathbf{z}_v^k)/\tau)}{\sum_{j\in\{v, v^\prime,v^{\prime\prime}\}}(\exp(s(\mathbf{z}_v^u, \mathbf{z}_v^k)/\tau)+\exp(s(\mathbf{z}_j^u, \mathbf{z}_v^k)/\tau))},
\end{equation}
where $v^\prime, v^{\prime\prime}$ are stochastically sampled negative candidates for item $v$. $s(\cdot)$ is the similarity measurement which we set to the cosine similarity of normalized vectors. $\tau$ is the temperature hyperparameter that controls the hardness~\cite{khosla2020supervised, sgl} of the contrastive goal.

\subsection{Model Learning and Discussion}
\subsubsection{\textbf{Joint Learning.}}
For the main recommendation task, the dot product between user and item representations $\hat{y}_{uv} = \mathbf{e}_u^\trans\mathbf{e}_v$ is used as the prediction. In line with baseline models~\cite{kgat,kgcl,kgin}, we adopt the widely used BPR~\cite{bpr} loss to optimize the model parameters as:
\begin{equation}
    \mathcal{L}_{rec} = \sum_{(u,v,j)\in\mathcal{D}}-\log\sigma\left(\hat{y}_{uv}-\hat{y}_{uj}\right),
\end{equation}
where $\mathcal{D} = \{(u,v,j)\}$ is the training instances with $v$ as the ground-truth and $j$ as the random sampled negative interaction. Note that we continue to adopt the entity embeddings $\mathbf{e}_v$ from masked graph $\mathcal{G}_k^m$ for the recommendation task, rather than performing aggregation on the original knowledge graph again. Since the masked triplets are generally of small size (\eg 512) compared to the whole graph (\eg millions), this trick affects little on the representation learning while greatly improves the training efficiency. According to~\cite{li2022scaling, he2022masked}, this setting can also increase the difficulty of the main task learning and thus lead to better gradients.

We optimize the all the loss in a joint learning manner to define the overall loss function:
\begin{equation}
    \mathcal{L} = \mathcal{L}_{rec} + \lambda_1\mathcal{L}_m + \lambda_2\mathcal{L}_c,
\end{equation}
where $\lambda_1, \lambda_2$ denote the weight of the mask\&reconstruction and cross-view contrastive learning task, separately. We omit the notation of L2 regularization terms for brevity.

\subsubsection{\textbf{Connection to Alignment and Uniformity.}}
To provide fundamental support for the proposed~\model~method, we investigate the alignment and uniformity merits that \model~brings on learned representations by the generative and contrastive tasks. Following~\cite{wang2020understanding, yu2022graph}, the mathematical definitions for the uniformity and alignment of learned vector representations are as:
\begin{align}
\mathcal{L}_{align} &\coloneqq \mathbb{E}_{(x,y)\sim p^+}[\|\mathbf{x}-\mathbf{y}\|_2^\alpha];\ \alpha>0\label{eq:au1}\\
\mathcal{L}_{uni}
&\coloneqq\log \mathbb{E}_{(x,y)\stackrel{i.i.d.}\sim p}[\exp(-\gamma\|\mathbf{x}-\mathbf{y}\|^2_2)];\ \gamma=1/2\sigma^2,\label{eq:au3}
\end{align}
where $\alpha$ denotes the exponent of the Euclidean distance. $p$ is the distribution of training data and $p^+$ is the distribution of positive labels. 

We first prove that the rational masking-reconstructing task is an explicit alignment for features. According to the generative loss in Equation~\ref{eq:mr}, the optimization of $\mathcal{L}_m$ equals to:
\begin{equation}
    \min\mathbb{E}_{(x,y)\sim p_r^+}\left[\sum_{x,y}\log\left(\sigma\left(\mathbf{x^\trans\mathbf{y}}\right)\right)\right],
\end{equation}
where $\mathbf{x}$ refers to head entity $\mathbf{e}_h$ and y to the element-wise product of tail entity and the relation: $\mathbf{e}_r\odot\mathbf{e}_t$. $p_r^+$ is the distribution of knowledge rationales with high rational scores. Note that:
\begin{equation}
\label{eq:align_trans}
    \|\mathbf{x}-\mathbf{y}\|_2^\alpha = (2-2\cdot\mathbf{x}^\trans\mathbf{y})^\frac{\alpha}{2}.
\end{equation}
Hence, $\mathcal{L}_m$ as the generative loss is in form of alignment as defined in Equation~\ref{eq:au1}. By optimizing $\mathcal{L}_m$, we force masked rational knowledge triplets to align as reconstruction.

We further derive the contrastive loss in Equation~\ref{eq:lc} to be reflective of the alignment and uniformity properties. Consider that:
\begin{align}
\label{eq:lc_au}
    \mathcal{L}_c &= \mathbb{E}_{\substack{(x,y)\sim p_c^+ \\ \{x_i^-\}_{i=1}^2\sim p_c}}\left[-\frac{1}{\tau}\mathbf{x}^\trans\mathbf{y} + \log\left(\exp(\mathbf{x}^\trans\mathbf{y}/\tau) + \sum_i\exp(\mathbf{{x_i^-}^\trans\mathbf{x}}/\tau) \right) \right]\\
\label{eq:lc_au_lb}    &\geq \mathbb{E}_{\substack{x\sim p_c \\ \{x_i^-\}_{i=1}^2\sim p_c}}\left[ -\frac{1}{\tau} + \log\left( \exp(\frac{1}{\tau}) + \sum_i\exp(\mathbf{{x_i^-}^\trans\mathbf{x}}/\tau) \right) \right]
\end{align}
where we denote the positive pair as $\mathbf{x},\mathbf{y}$ and negative samples as $\mathbf{x^-}$ for brevity. $\{x_i^-\}_{i=1}^2\sim p_c$ is the set of random negative samples in Equation~\ref{eq:lc}, and $p_c$ denotes the distribution of cross-view item representations. Therefore, the lower bound of $\mathcal{L}_c$ in Equation~\ref{eq:lc_au_lb} is satisfied if and only if the embeddings $\mathbf{x},\mathbf{y}$ is perfectly aligned as $\mathbf{x}^\trans\mathbf{y}=1$, equivalent to the definition of alignment in Equation~\ref{eq:au1}. Suppose that the embeddings satisfy the perfect alignment condition, the optimization of $\mathcal{L}_c$ degenerates to:
\begin{align}
    \min\mathbb{E}_{\substack{x\sim p_c \\ \{x_i^-\}_{i=1}^2\sim p_c}}\left[\log\left(\sum_i\exp(\mathbf{{x_i^-}^\trans\mathbf{x}}/\tau)\right)\right],
\end{align}
which satisfies the objective in Equation~\ref{eq:au3} as the uniformity loss. Hence, the alignment and uniformity merits in $\mathcal{L}_m$ and $\mathcal{L}_c$ can benefit the representation learning, by forcing the agreement between positive pairs and pushing random instances as negatives. Furthermore, the proposed knowledge rationalization mechanism improves the sampling distribution to be rational: $p_r^+$, and noise-free: $p_c^+$, instead of the widely-used random distribution $p$ in the original forms. By exploiting rationales in the KG considering the contribution to recommendation, we empower the alignment property with rationality-aware positive pairing ability, which provides better gradients for model learning. Additionally, for the cross-view rationales, we remove potential noise to build noise-free distribution $p_c$, which eliminates the effect of false negative pairing to improve contrastive effectiveness. Overall, our \model~is able to derive better alignment and uniformity, comparing to stochastic methods.

% To this end, we say $\mathcal{L}_c$ has the alignment and uniformity properties that benefit the representation learning. And obviously, referring to Equation~\ref{eq:align_trans}, the masking-reconstructing loss $\mathcal{L}_m$ is directly forcing the alignment property of entity representations with relational context.

% Comprehensively, by self-supervision regularization $\mathcal{L}_m$ and $\mathcal{L}_c$, we achieve the alignment goal by forcing the agreement between semantically positive pairs, \ie masked knowledge rationales and cross-view representations of identical items. By further exploiting rationales in the KG considering contribution to recommendation, we empower the alignment property with rationality-aware positive pairing ability. Specifically, the proposed rational knowledge masking and rationalized cross-view augmentation can enhance the accurateness of the alignment goal by generating positive pairs that are noise-free and intuitive for the recommendation task. And for information maximization, the uniformity property of $\mathcal{L}_c$ forces the uniform distribution of feature embeddings to improve the discrimination between representations.
